Efficient Regex Matching with Sparse Counting-Sets

Regular expressions with counting operations (c-regexes) offer a compact representation of repeating patterns by allowing numerical bounds to be added to subexpressions. Recent work introduced the counting-set data structure, which allows simultaneous updates of multiple counter values for efficient matching. However, this approach suffers from a performance bottleneck when counting-sets must be replicated due to the presence of branching transitions. We propose a sparse counting-set approach, which reduces the replication overhead by maintaining only essential counter values, thereby yielding a more efficient matching algorithm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{C. C\^{a}mpeanu, M. Kutrib, S. Lombardy (Eds.) \\
Non-Classical Models of Automata and Applications (NCMA 2026)\\
EPTCS 446, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.446.2}{10.4204/EPTCS.446.2}}
\pdfoutput=1

